INN-PAR: Invertible Neural Network for PPG to ABP Reconstruction

Non-invasive and continuous blood pressure (BP) monitoring is essential for the early prevention of many cardiovascular diseases. Estimating arterial blood pressure (ABP) from photoplethysmography (PPG) has emerged as a promising solution. However, existing deep learning approaches for PPG-to-ABP reconstruction (PAR) encounter certain information loss, impacting the precision of the reconstructed signal. To overcome this limitation, we introduce an invertible neural network for PPG to ABP reconstruction (INN-PAR), which employs a series of invertible blocks to jointly learn the mapping between PPG and its gradient with the ABP signal and its gradient. INN-PAR efficiently captures both forward and inverse mappings simultaneously, thereby preventing information loss. By integrating signal gradients into the learning process, INN-PAR enhances the network's ability to capture essential high-frequency details, leading to more accurate signal reconstruction. Moreover, we propose a multi-scale convolution module (MSCM) within the invertible block, enabling the model to learn features across multiple scales effectively. We have experimented on two benchmark datasets, which show that INN-PAR significantly outperforms the state-of-the-art methods in both waveform reconstruction and BP measurement accuracy. Codes can be found at: https://github.com/soumitra1992/INNPAR-PPG2ABP.

==> 2_method/eqn_mscn.tex <==
\begin{align}
\begin{split}
X_f^1 & = \sigma(W(X_i^1)) \in \mathbb{R}^{L \times C}\:;\:
X_i^2 = DS(X_f^1) \in \mathbb{R}^{\frac{L}{2} \times 2C}\\
X_f^2 & = \sigma(W(X_i^2)) \in \mathbb{R}^{\frac{L}{2} \times 2C}\:;\:
X_i^3 = DS(X_f^2) \in \mathbb{R}^{\frac{L}{4} \times 4C}\\
X_f^3 & = \sigma(W(X_i^3)) \in \mathbb{R}^{\frac{L}{4} \times 4C}\:;\:
X_i^{'2} = US(X_f^3) \in \mathbb{R}^{\frac{L}{2} \times 2C}
\\
X_f^{'2} & = \sigma(W(X_i^{'2})) \in \mathbb{R}^{\frac{L}{2} \times 2C}\:;\:
X_i^{'1} = US(X_f^{'2}) \in \mathbb{R}^{L \times C}\\
X_o^1 & = W(X_i^{'1}) \in \mathbb{R}^{L \times 1}
\end{split}
\end{align}

where $\sigma(\cdot)$ denotes ReLU activation function, $W(\cdot)$ is convolution operation. $X_f^k$, $X_f^{'k}$, $X_i^k$, and $X_i^{'k}$ are the features and inputs at $k^{th}$ scale. $DS(\cdot)$ and $US(\cdot)$ denote downscaling and upscaling operations respectively. 

==> images/fig3.tex <==
\begin{figure*}[hbt!] 
   \begin{subfigure}[t]{0.495\columnwidth}
    \includegraphics[width=\linewidth]{images/ppg.png}
    \caption{PPG Signal}
    \label{fig:1}
  \end{subfigure}
  \hfill %%
  \begin{subfigure}[t]{0.495\columnwidth}
    \includegraphics[width=\linewidth]{images/unet.png}
    \caption{UNet1d}
    \label{fig:2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.495\columnwidth}
    \includegraphics[width=\linewidth]{images/vnet.png}
    \caption{VNet1d}
    \label{fig:1}
  \end{subfigure}
  \hfill %%
  \begin{subfigure}[t]{0.495\columnwidth}
    \includegraphics[width=\linewidth]{images/lista.png}
    \caption{INPAR (Ours)}
    \label{fig:2}
  \end{subfigure}
     \begin{subfigure}[t]{0.495\columnwidth}
    \includegraphics[width=\linewidth]{images/ppg.png}
    \caption{PPG Signal}
    \label{fig:1}
  \end{subfigure}
  \hfill %%
  \begin{subfigure}[t]{0.495\columnwidth}
    \includegraphics[width=\linewidth]{images/unet.png}
    \caption{UNet1d}
    \label{fig:2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.495\columnwidth}
    \includegraphics[width=\linewidth]{images/vnet.png}
    \caption{VNet1d}
    \label{fig:1}
  \end{subfigure}
  \hfill %%
  \begin{subfigure}[t]{0.495\columnwidth}
    \includegraphics[width=\linewidth]{images/lista.png}
    \caption{INPAR (Ours)}
    \label{fig:2}
  \end{subfigure}
  \caption{Visual comparison with SOTA methods. The first row shows a signal from the Sensors dataset \cite{sensors}, and the second row shows a signal from the BCG dataset \cite{bcg}.}
  \label{fig3} 
\end{figure*}

==> images/fig4.tex <==
\begin{figure}[htb]
  \begin{subfigure}[t]{0.48\columnwidth}
    \includegraphics[width=\linewidth]{images/design.png}
    \caption{Design Settings (DS)}
    \label{fig:1}
  \end{subfigure}
  \hfill %%
  \begin{subfigure}[t]{0.48\columnwidth}
    \includegraphics[width=\linewidth]{images/loss.png}
    \caption{Loss Settings (LS)}
    \label{fig:2}
  \end{subfigure}
  \caption{Ablation experiments with different settings.}
  \label{fig4}
\end{figure}




==> sec/0_abstract.tex <==
\begin{abstract}
Routine monitoring of blood pressure (BP) is important to prevent cardiac diseases. Photoplethysmography (PPG) to arterial blood pressure (ABP) estimation provides a non-invasive technique for continuous monitoring of BP. Recently proposed
deep learning-based methods have achieved impressive results
in PPG to ABP reconstruction (PAR) task. However, these methods often cause
significant information loss about the input PPG signal. To
address this issue, we introduce an invertible neural network for PAR (INN-PAR). Using a series of invertible blocks, INN-PAR jointly learns the mapping between PPG and its gradient with those of the ABP signal. Specifically, we propose a multi-scale convolution module in the invertible block for learning features at multi-scales.
Our experiments show that INN-PAR surpasses state-of-the-art methods in performance. 
\\
\\
\\
Models and code can be found at the following link: [Link]
\end{abstract}

\begin{IEEEkeywords}
PPG, ABP, waveform reconstruction, invertible network.
\end{IEEEkeywords}

==> sec/1_intro.tex <==
\input{images/fig1}
\section{Introduction}
\label{sec:intro}
Blood pressure (BP) is a crucial biomarker for early detection of cardiovascular diseases. Therefore, routine BP monitoring is of utmost importance to prevent premature death. Traditional BP monitoring methods can be divided into two categories: invasive continuous monitoring of arterial blood pressure (ABP), and non-invasive wrist cuff-based measurement. Compared to the invasive ABP measurement, cuff-based BP monitoring is more convenient. However, the cuff-based method cannot continuously monitor the BP since it is unrealistic to continuously perform cuff inflations and deflations.  Photoplethysmography (PPG), which can continuously measure the volumetric variations of blood circulation, is a potential alternative to monitor BP non-invasively and continuously \cite{nature}. 

In recent years, a number of works \cite{icassp2,icassp3,icassp4,icassp5,icassp6, sensors,vnet,unet1} have been proposed for PPG-based BP monitoring. Among these, few works \cite{sensors,vnet,unet1} proposed deep learning-based methods to estimate the ABP waveform from the PPG signal. From the estimated ABP signal, the systolic blood pressure (SBP) and diastolic blood pressure (DBP) can be measured by identifying the systolic peaks onset and offset of each cardiac cycle. The PPG to ABP reconstruction methods \cite{sensors,vnet,unet1} follow two steps: feature extraction and signal reconstruction. Though these methods are effective for the PAR task, during the feature extraction stage, significant information is lost about the input PPG signal due to the non-injective mapping learned by the network. Moreover, these methods did not consider the signal gradient, which contains significant structural information about the signal.

To address the information loss issue in PAR task, invertible neural network (INN) \cite{nice} can be used. INN learns a series of invertible bijective transformations to learn the mapping between input $x$ and output $y$ as,

\begin{align}
\begin{split}
y & = f_0\circ f_1\circ f_2\circ \dots \circ f_N (x) \\
x & = f_0^{-1}\circ f_1^{-1}\circ f_2^{-1}\circ \dots \circ f_N^{-1} (y)
\end{split}
\end{align}

where $\{f_k\}_{k=0}^N$ are invertible and bijective functions. Though INN is mainly used for generative tasks in the image \cite{nice,realnvp,glow} and signal processing \cite{waveglow,speech} domain, several prior works used INN for image reconstruction tasks \cite{rescaling,icassp7}. For PPG to ABP waveform reconstruction, INN framework can be effective as it does not discard any information about the input PPG signal. Moreover, for the PAR task, considering the learning of signal gradient mapping can be highly effective. 

This work proposes an invertible network for PPG to ABP reconstruction (INPAR), that uses a stack of invertible blocks for the PAR task. While learning the mapping between PPG and ABP, INPAR also learns the mapping between their gradients. This gradient learning helps in reconstructing the high-frequency details with better accuracy. Also, we introduce a multi-scale convolution module (MSCM) in the invertible block of INPAR for learning multi-scale features. While training INPAR, we constrain the estimated ABP and its gradient to be similar with those of the ground truth ABP signal, Extensive experiments across two benchmark datasets demonstrate that INPAR surpasses the state-of-the-art methods in waveform reconstruction and SBP and DBP measurement accuracies.
 
The rest of this paper is organized as follows. In Section \ref{sec:method}, we describe the architecture of INPAR and the loss function. Section \ref{sec:experiments} presents extensive experiments to validate the effectiveness of our proposed method. Finally, Section \ref{sec:conclusion} concludes the paper.


==> sec/1_intro1.tex <==
\input{images/fig1}
\section{Introduction}
\label{sec:intro}
Continuous blood pressure monitoring is essential for the early detection and management of several cardiovascular diseases. Blood pressure measurement provides critical insights into the dynamic nature of cardiovascular function, reflecting the intricate balance between cardiac output (the volume of blood pumped by the heart) and vascular resistance (the force opposing blood flow in the vessels). Systolic blood pressure (SBP), the higher of the two values, signifies the peak pressure in the arteries during the heart's contraction, while diastolic blood pressure (DBP) indicates the minimum pressure during the heart's resting phase between beats.

Traditional methods of measuring blood pressure can be divided into invasive and non-invasive techniques. Invasive methods, which involve arterial cannulation, pose serious risks, while non-invasive methods like cuff-based sphygmomanometers offer a safer, more convenient alternative. However, these cuff-based devices are often bulky and impractical for continuous monitoring due to the need for repeated cuff inflations and deflations.

To address these limitations, photoplethysmography (PPG) has emerged as a promising technique for non-invasive continuous blood pressure monitoring. PPG measures the volumetric variations of blood circulation and can potentially provide continuous blood pressure data.

Recent advancements in BP estimation have explored a range of techniques, from traditional feature-based statistical methods to deep learning approaches. Feature-based methods rely on predefined sets of features, which can restrict the amount of information retained from the input signal. In contrast, deep learning methods address these limitations by generating signal embeddings that capture more detailed input data. BP estimation often involves analyzing arterial blood pressure (ABP) waveforms, which allow for the determination of systolic (SBP) and diastolic (DBP) pressures through the identification of systolic peak onset and offset in each cardiac cycle.

Ibtehaz et al. proposed a cascade-based deep learning approach, PPG2ABP, that normalizes raw PPG and ABP waveforms. This method initially estimates the ABP waveform using an Approximation Network and refines it with a Refinement Network. While the method delivered promising performance, it did not consistently maintain the shape of the ABP waveform. To address this, Mahmud et al. introduced NABNet, a hybrid model aimed at reducing errors caused by phase lag in ABP during segmentation.

Despite the effectiveness of these deep learning methods in reconstructing PPG-to-ABP signals, significant information loss still occurs, primarily due to the non-injective mapping inherent in the feature extraction process.

To address the information loss issue in PAR task, invertible neural network (INN) \cite{nice} can be used. INN learns a series of invertible bijective transformations to learn the mapping between input $x$ and output $y$ as,

\begin{align}
\begin{split}
y & = f_0\circ f_1\circ f_2\circ \dots \circ f_N (x) \\
x & = f_0^{-1}\circ f_1^{-1}\circ f_2^{-1}\circ \dots \circ f_N^{-1} (y)
\end{split}
\end{align}

where $\{f_k\}_{k=0}^N$ are invertible and bijective functions. Though INN is mainly used for generative tasks in the image \cite{nice,realnvp,glow} and signal processing \cite{waveglow,speech} domain, several prior works used INN for image reconstruction tasks \cite{rescaling,icassp7}. For PPG to ABP waveform reconstruction, INN framework can be effective as it does not discard any information about the input PPG signal. Moreover, for the PAR task, considering the learning of signal gradient mapping can be highly effective. 

This work proposes an invertible network for PPG to ABP reconstruction (INPAR), that uses a stack of invertible blocks for the PAR task. While learning the mapping between PPG and ABP, INPAR also learns the mapping between their gradients. This gradient learning helps in reconstructing the high-frequency details with better accuracy. Also, we introduce a multi-scale convolution module (MSCM) in the invertible block of INPAR for learning multi-scale features. While training INPAR, we constrain the estimated ABP and its gradient to be similar with those of the ground truth ABP signal, Extensive experiments across two benchmark datasets demonstrate that INPAR surpasses the state-of-the-art methods in waveform reconstruction and SBP and DBP measurement accuracies.
 
The rest of this paper is organized as follows. In Section \ref{sec:method}, we describe the architecture of INPAR and the loss function. Section \ref{sec:experiments} presents extensive experiments to validate the effectiveness of our proposed method. Finally, Section \ref{sec:conclusion} concludes the paper.

==> sec/4_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This work proposes INN-PAR, an invertible network for the PAR task. Different from other deep learning-based methods, our network has an information lossless architecture. INN-PAR jointly learns the mapping between the PPG and its gradient with those of the ABP signal. Our ablation experiments justify the design of INN-PAR. Extensive experiments demonstrate that INN-PAR outperforms state-of-the-art methods. Future work could explore invertible network designs further, considering different deep-learning architectures to improve the accuracy of the PAR task.
